Aggregation and Embedding for Group Membership Verification

This paper proposes a group membership verification protocol preventing the curious but honest server from reconstructing the enrolled signatures and inferring the identity of querying clients. The protocol quantizes the signatures into discrete embeddings, making reconstruction difficult. It also aggregates multiple embeddings into representative values, impeding identification. Theoretical and experimental results show the trade-off between the security and the error rates.

==> BloomFilter.tex <==
% !TEX root = GroupMembershipVerification.tex

\appendix
\section{A baseline based on Bloom Filter}
\label{sec:BloomFilter}
%{\color{red} This section is just a note for the moment.}

This section presents a baseline based on Bloom filter.
This data structure is meant for group membership but for discrete objects.
For this reason, at the enrollment and the query time, vectors are first quantized by a similar Ternary Sparse coding:
% and passed to the Bloom filter:
$\func{h}: \real^{\dim}\to \{-1,0, +1\}^{\ell}$
with $\func{h}(\x)_{i} = \func{sign}(\w_{i}^{\top}\x)\un_{>\lambda}(|\w_{i}^{\top}\x|)$.

We denote by $H(\lambda,\ell)$ the entropy of the output $\func{h}(\X)$, $\pi_{0}(\lambda,\ell)$ the probability to be quantized onto $\0_{\ell}$, and $\pi(\lambda,\ell) = \Pr(\func{h}(\x+\n) = \func{h}(\x))$, where $\n$ is a Gaussian white noise of a given variance $\sigma_{n}^{2}$. It easily comes that:
\begin{eqnarray}
H(\lambda,\ell)&=&\ell \left(-2p\log(2p) - (1-2p)\log(1-2p) \right),\\
\pi_{0}(\lambda,\ell) &= &(1-2p)^{\ell}\\
\pi(\lambda,\ell) &=& p_{s}^{\ell},\quad\text{with}\\
%\end{eqnarray}
%\begin{eqnarray}
%p&:=& \Phi(-\lambda/\sigma_{x}),\quad \text{and}\\
p&:=& \Phi_{\sigma_{x}}(-\lambda),\quad \text{and}\\
%p_{s}&:=&2\int_{\lambda}^{+\infty} \phi(x) \left(1-\Phi\left(-\frac{\lambda+x}{\sigma_{n}}\right)\right)dx\nonumber\\
%&+&\int_{-\lambda}^{\lambda} \phi(x) \left(\Phi\left(\frac{\lambda-x}{\sigma_{n}}\right) - \Phi\left(-\frac{\lambda+x}{\sigma_{n}}\right)\right) dx\nonumber
p_{s}&:=&2\int_{\lambda}^{+\infty} \phi_{\sigma_{x}}(x) \left(1-\Phi_{\sigma_{n}}\left(-\lambda-x\right)\right)dx\nonumber\\
&+&\int_{-\lambda}^{\lambda} \phi_{\sigma_{x}}(x) \left(\Phi_{\sigma_{n}}\left(\lambda-x\right) - \Phi_{\sigma_{n}}\left(-\lambda-x\right)\right) dx.\nonumber
\end{eqnarray}
where $\phi_{\sigma}$ and $\Phi_{\sigma}$ are the density and cumulative density functions of a Gaussian variable with variance $\sigma^{2}$.
Whenever $\func{h}(\x+\n) \neq \func{h}(\x)$, the Bloom filter does not deem $\x+\n$ as a version of $\x$.
This happens with probability $1-\pi(\lambda,\ell)$.

The theory of Bloom filter helps designing this data structure.
Its optimal length is given by
\begin{equation}
\ell_{B}=\lceil N|\log \pfp|\log(2)^{-2} \rceil.
\label{eq:LengthBF}
\end{equation}
The quantized vector feeds a series of hashed functions, which output random indices in $\{1,\ldots,\ell_{B}\}$.
These indices must be uniformly distributed with entropy $\log(\ell_{B})$.
We assume there exist such hashing functions provided that the entropy of the quantized vectors is bigger than $\log(\ell_{B}) + h$, where $h$ is an entropy margin. We also want that none of the $N$ enrolled signatures are quantized to 0 with probability $1-\epsilon$, which implies $\pi_{0}(\lambda,\ell)<\epsilon/N$.

Then, we solve the following problem numerically:
\begin{equation}
(\lambda,\ell) = \arg\max_{H(\lambda,\ell) > \log(\ell_{B}) + h, \pi_{0}(\lambda,\ell)<\epsilon/N} \pi(\lambda,\ell).
\end{equation}
Fig.~\ref{fig:compare} and~\ref{fig:AUCN} use this optimal setting with $h=3$ nats and $\epsilon=10^{-3}$.


==> Collecting.tex <==
Our goal is finding a representative for each group of data, i.e. a group of vectors $\mathcal{G}=\{\textbf{x}_{1},\textbf{x}_{2},...,\textbf{x}_{m}\}$aggregated into one vector $\textbf{x}_{\mathcal{G}}$. Based on aggregation is applied in original domain or code domain, we can define two baselines. 
\subsection{Baseline 1}
\label{Baseline 1}
All members of a group  can be aggregated into one vector with the same dimension
and then the group representative $\textbf{x}_{\mathcal{G}}$ obtained by computing the signature of aggregated vector. Let $f:\mathbb{R}^{N\times m}\rightarrow \mathbb{R}^{N}$ be the aggregation function, $h:\mathbb{R}^{N}\rightarrow \mathbb{R}^{l}$ the hash function and $\textbf{G}=[\textbf{x}_1,...,\textbf{x}_m]$, the representative $\textbf{x}_{\mathcal{G}}$ for a group of vectors $\mathcal{G}$ is defined as
$h(\mathit{f}(\textbf{G}))$, where we produce the signatures by ternary sparse coding, i.e., $h(\textbf{x})=T_{\lambda_x}(\textbf{Wx})$.
\subsection*{Aggregation by sum}
A simple aggregation function can be defined as sum of the vectors in a group, i.e. 
$\mathit{f}(\textbf{G})=\sum_{i=1}^{m}\textbf{x}_i$.
\subsection*{Aggregation by pseudo inverse}
We use strategy of designing memory vector proposed by Ahmet et al. \cite{memoryvector}, which aims to optimize the construction of aggregated vector $\textbf{f}=\mathit{f}(\textbf{G})$, where $\textbf{G}=[\textbf{x}_1,...,\textbf{x}_m]$. Assume all vectors are normalizer to have  unit norm, i.e., $||\textbf{x}||_2^2=1$, Minimizing the squared $L_2$-norm of $\textbf{f}$, i.e. $||\textbf{f}||^2$ by constraining $\textbf{x}_i^T\textbf{f}=1, \forall i\in{1,...,m}$ leads to the solution $\textbf{f}^*=(\textbf{G}^+)^T\textbf{1}_m$, where $\textbf{G}^+$ is pseudo-inverse of $\textbf{G}$ and $\textbf{1}_m$ denotes a length $m$ vector with all entries one.


\subsection{Baseline 2}
\label{Baseline 2}
Unlike the first baseline which has the strategy of "Aggregation+Embedding", where group members are aggregated in original domain, we can have the strategy of "Embedding+Aggregation", so the aggregation will happen in transform domain.\\
Given the hash function $h:\mathbb{R}^{N}\rightarrow \mathbb{R}^{l}$ and aggregation function $f:\mathbb{R}^{l\times m}\rightarrow \mathbb{R}^{l}$, the representative for a group $\mathcal{G}=\{\textbf{x}_1,...,\textbf{x}_m\}$ computed as $f([\mathit{h}(\textbf{x}_1),...,\mathit{h}(\textbf{x}_m)])$.


\subsection*{Aggregation by sum pooling}
Sparse ternary coding is used as the hash function $h:\mathbb{R}^{N}\rightarrow \{-1,0,+1\}^{l}$. In this way, for a set of vectors the mid level coding of each vector can be expressed as $\textbf{a}_i=T_{\lambda_x}(\textbf{Wx}_i), \forall i\in{1,...,m}$. 
Now the group signature can be represented by summing over all the signatures of group and applying the sign function to the resultant vector, i.e., $sign(\sum_{i=1}^{m}\textbf{a}_i)$.

\subsection*{Aggregation by majority voting}
The other method for pooling the vectors can be done through majority voting. To this end, after computing the mid level coding, for each element, we can pick up the most frequently value among $\{-1,0,+1\}$, i.e. the $i$-th component of group representation obtained as $mode(\textbf{a}_{1_i},...,\textbf{a}_{m_i})$, where $\textbf{a}_{j_i}$ corresponds to $i$-th element of signature of $\textbf{x}_j$.

==> Encoding.tex <==
%The encoding process for enrollment stage has two steps. We assume that each data sample belongs to only one group, so at the first step each data sample is assigned to a group, then for each group all vectors are collected to produce the group representation.

%\subsection{Partitioning}
%\label{Partitioning}
%For partitioning, we consider 3 scenarios:
%\begin{itemize}
%	\item Random assignment: The database vectors are randomly assigned into $k$ groups and all of them have the same size, i.e., $m_i=\frac{M}{k},  \forall i\in{1,...,k}$.
%	\item Clustering: The assignments can be done in a manner such that similar vectors assigned to groups.
%	\item Anti-Clustering: The vectors packed in the same group are as far apart as possible.
%\end{itemize}
%\subsubsection*{Clustering}	
%	For this purpose, clustering algorithms such as $k$-means can be utilized, where this algorithm intends to partition data into $k$ clusters in which each object belongs to the cluster with the nearest mean. Since, the objective of $k$-means clustering is to minimize the inter-cluster similarity and maximize the intra-cluster similarity ,this method produces k different clusters of greatest possible distinction. 
%\subsubsection*{Anti-Clustering}	
%Unlike clustering algorithms, we aim to find groups such that vectors assigned to groups are not similar to each other at all.\\
%Inspired by the idea of hierarchical agglomerative clustering, we define each data point as a group and at each step merge two groups that have largest distance and continue merging until the number of groups equals $k$.

%\subsection{Collecting}
%\label{Collecting}
%Our goal is finding a representative for each group of data, i.e. a group of vectors $\mathcal{G}=\{\textbf{x}_{1},\textbf{x}_{2},...,\textbf{x}_{m}\}$aggregated into one vector $\textbf{x}_{\mathcal{G}}$. Based on aggregation is applied in original domain or code domain, we can define two baselines. 
%\subsubsection{Baseline 1}
%\label{Baseline 1}
%All members of a group  can be aggregated into one vector with the same dimension
%and then the group representative $\textbf{x}_{\mathcal{G}}$ obtained by computing the signature of aggregated vector. Let $f:\mathbb{R}^{N\times m}\rightarrow \mathbb{R}^{N}$ be the aggregation function, $h:\mathbb{R}^{N}\rightarrow \mathbb{R}^{l}$ the hash function and $\textbf{G}=[\textbf{x}_1,...,\textbf{x}_m]$, the representative $\textbf{x}_{\mathcal{G}}$ for a group of vectors $\mathcal{G}$ is defined as
%$h(\mathit{f}(\textbf{G}))$, where we produce the signatures by ternary sparse coding, i.e., $h(\textbf{x})=T_{\lambda_x}(\textbf{Wx})$.
%\subsubsection*{Aggregation by sum}
%A simple aggregation function can be defined as sum of the vectors in a group, i.e. 
%$\mathit{f}(\textbf{G})=\sum_{i=1}^{m}\textbf{x}_i$.
%\subsubsection*{Aggregation by pseudo inverse}
%We use strategy of designing memory vector proposed by Ahmet et al. \cite{memoryvector}, which aims to optimize the construction of aggregated vector $\textbf{f}=\mathit{f}(\textbf{G})$, where $\textbf{G}=[\textbf{x}_1,...,\textbf{x}_m]$. Assume all vectors are normalized to have  unit norm, i.e., $||\textbf{x}||_2^2=1$, minimizing the squared $L_2$-norm of $\textbf{f}$, i.e. $||\textbf{f}||^2$ by constraining $\textbf{x}_i^T\textbf{f}=1, \forall i\in{1,...,m}$ leads to the solution $\textbf{f}^*=(\textbf{G}^+)^T\textbf{1}_m$, where $\textbf{G}^+$ is pseudo-inverse of $\textbf{G}$ and $\textbf{1}_m$ denotes a length $m$ vector with all entries one.
%
%
%\subsubsection{Baseline 2}
%\label{Baseline 2}
%Unlike the first baseline which has the strategy of "Aggregation+Embedding", where group members are aggregated in original domain, we can have the strategy of "Embedding+Aggregation", so the aggregation will happen in transform domain.\\
%Given the hash function $h:\mathbb{R}^{N}\rightarrow \mathbb{R}^{l}$ and aggregation function $f:\mathbb{R}^{l\times m}\rightarrow \mathbb{R}^{l}$, the representative for a group $\mathcal{G}=\{\textbf{x}_1,...,\textbf{x}_m\}$ computed as $f([\mathit{h}(\textbf{x}_1),...,\mathit{h}(\textbf{x}_m)])$.
%
%
%\subsubsection*{Aggregation by sum pooling}
%Sparse ternary coding is used as the hash function $h:\mathbb{R}^{N}\rightarrow \{-1,0,+1\}^{l}$. In this way, for a set of vectors the mid level coding of each vector can be expressed as $\textbf{a}_i=T_{\lambda_x}(\textbf{Wx}_i), \forall i\in{1,...,m}$. 
%Now the group signature can be represented by summing over all the signatures of group and applying the sign function to the resultant vector, i.e., $sign(\sum_{i=1}^{m}\textbf{a}_i)$.
%
%\subsubsection*{Aggregation by majority voting}
%The other method for pooling the vectors can be done through majority voting. To this end, after computing the mid level coding, for each element, we can pick up the most frequently value among $\{-1,0,+1\}$, i.e. the $i$-th component of group representation obtained as $mode(\textbf{a}_{1_i},...,\textbf{a}_{m_i})$, where $\textbf{a}_{j_i}$ corresponds to $i$-th element of signature of $\textbf{x}_j$.



==> Experiments.tex <==
% !TEX root = GroupMembershipVerification.tex

\section{Experiments}
\label{sec:Experiments}

In this section, we conduct experiments on synthetic data, by generating $M=$ 8192 i.i.d. random vectors from the normal distribution with zero mean and variance $\sigma^2_x$  in $N=$ 256 dimensional space. We consider the dimension of signatures as $L=N$.
For a query $\textbf{y}$, to perform a test
and answer the question whether "$\textbf{y}$ is related to our database?", we compare it with all group representations. Then area under receiver operating characteristic (ROC) curve AUC is used as a performance measure.
Fig.~\ref{fig:Fig.1} illustrates performance of aggregation methods described in Section \ref{Collecting} by three different partitioning strategies. Since, in aggregation by pseudo inverse, we assumed that each vector has a unit norm, in Fig.~\ref{Fig.1}.b we normalize each vector in database to have a length of one and then perform group embedding.

\begin{figure}%	
	\centering
	\includegraphics[width=0.5\linewidth]{Figs/fig1_a_randomSx2.pdf}
	\includegraphics[width=0.5\linewidth]{Figs/fig1_b_randomSx2.pdf}
	%\subfloat[]{{\includegraphics[width=5cm]{Figs/fig1_a_randomSx2.pdf} }}%
	%\qquad
	%\subfloat[]{{\includegraphics[width=5cm]{Figs/fig1_b_randomSx2.pdf} }}%
	\caption{The performance of different aggregation and partitioning methods.}%
	\label{fig:Fig.1}%
\end{figure}

In Fig.~\ref{fig:Fig.2}, an experiment is carried out to assess the influence of sparsity level $S_x$ on robustness of our group embedding method. %For this experiment, the partitioning is clustering and
\begin{figure}%	
	\centering
	\includegraphics[width=\linewidth]{Figs/fig2_Sx2.pdf}
	\caption{Impact of parameter $S_x$.}%
	\label{fig:Fig.2}%
\end{figure}
%\begin{figure}%
%	
%	\centering
%	\subfloat[]{{\includegraphics[width=5cm]{Figs/fig11_a_randomSx2.pdf} }}%
%	\qquad
%	\subfloat[]{{\includegraphics[width=5cm]{Figs/fig11_b_randomSx2.pdf} }}%
%	\caption{The performance of different aggregation and partitioning methods.}%
%	\label{Fig.3}%
%\end{figure}



Fig \ref{fig:Fig.4} depicts the difference between two formulas presented in Section \ref{Section4} to estimate the test statistics of group membership verification.



\begin{figure}%
	\centering
	\includegraphics[width=\linewidth]{Figs/fig3.pdf}
	\caption{Comparison between theoretical and experimental AUC of k groups.}%
	\label{fig:Fig.4}%
\end{figure}

\begin{figure}%
	\centering
	\includegraphics[width=\linewidth]{Figs/fig4.pdf}
	\caption{Random transformation vs. learned transformation.}%
	\label{fig:Fig.5}%
\end{figure}


==> MembershipVerification.tex <==
%In statistical hypothesis testing, a type I error, also known as “false positive”, is the rejection of a null hypothesis $\mathcal{H}_0$ when it is actually true, while a type II error, also known as "false negative", is the error of incorrectly reject the alternative hypothesis $\mathcal{H}_1$.
%Our problem is a group membership verification, which needs $k$(the number of groups) tests. In this section, we present two approaches for combining tests, to estimate the overall type I and II errors of our group testing problem.\\
%Suppose that the database containing $M$ vectors is packed into $k$ groups of size $m$. Let $\textbf{x}_{\mathcal{G}_1},...,\textbf{x}_{\mathcal{G}_k}$ be the group representations. For a query vector $\textbf{y}$, we perform $k$ tests and combine them. The combination of tests are in a parallel manner, which means that a test is positive if at least one of the tests are positive and it's negative if all the tests are negative.
%\subsection*{Individual tests}
%Given a query $\textbf{y}$, for $i$-th test, the corresponding hypotheses can be defined as:
%\begin{itemize}
%	\item hypothesis $\mathcal{H}_0$: \textbf{y} is not related to any vectors in the group.
%	\item hypothesis $\mathcal{H}_1$: \textbf{y} is related to at least one vector in $\mathcal{G}_i$, i.e., $\exists j \in \{1,...,m_i\}$, where $\textbf{y}=\textbf{x}_{ij}+\textbf{z}$.
%\end{itemize}
%Testing the membership of query \textbf{y} to $i$-th group can be done by thresholding $ \textit{similarity}(\textbf{y},\textbf{x}_{\mathcal{G}_i})$.\\
%Consider $P_{FP_i}(m,1)$ and $P_{FN_i}(m,1)$ as the false positive rate and false negative rate of $i$-th test ($(m,1)$ implies that for each test, the members of corresponding group are considered as positive observations). Now the false positive rate of combination of them, i.e. $P_{FP}(M,k)$ is the probability that at least one of the tests is positive, when the query isn't related to any group:\\
%$P_{FP}(M,k)=1-\prod_{i=1}^{k}P_{FP_i}(m,1)$\\
%The false negative rate of combination of tests, i.e. $P_{FN}(M,k)$ is the probability that all the tests are negative, when the query actually belongs to a group, so if it belongs to the $i$-th group, a false negative for this group and true negative for other groups occur:\\
%$P_{FN}(M,k)=\frac{1}{k}\sum_{i=1}^{k}P_{FN_i}(m,1)\prod_{j\neq i}P_{TN_j}(m,1)$.\\
%\subsection*{Parallel tests}
%The hypotheses of $i$-th test can be defined as:
%\begin{itemize}
%	\item hypothesis $\mathcal{H}_0$: \textbf{y} is not related to any vectors in the database.
%	\item hypothesis $\mathcal{H}_1$: \textbf{y} is related to at least one vector in $\mathcal{G}_i$, i.e., $\exists j \in \{1,...,m_i\}$, where $\textbf{y}=\textbf{x}_{ij}+\textbf{z}$.
%\end{itemize}
%To this end, for each test, we consider all the vectors in database as the positive observations.
%Let $P_{FP_i}(M,1)$ and $P_{FN_i}(M,1)$ be the false positive rate and false negative rate of $i$-th test ($(M,1)$ implies that all the database vectors are considered as positive observations). Since the tests are independent, the false positive rate of combination of them, i.e. $P_{FP}(M,k)$ is:\\
%$P_{FP}(M,k)=1-\prod_{i=1}^{k}P_{FP_i}(M,1)$\\
%The false negative rate of combination of tests, i.e. $P_{FN}(M,k)$ is the probability that all the tests are negative, when the query is related to database:\\
%$P_{FN}(M,k)=\prod_{i=1}^{k}P_{FN_i}(M,1)$.\\

